A joint optimization approach of parameterized quantum circuits with a tensor network

Despite the advantage quantum computers are expected to deliver when performing simulations compared to their classical counterparts, the current noisy intermediate-scale quantum (NISQ) devices remain limited in their capabilities. The training of parameterized quantum circuits (PQCs) remains a significant practical challenge, exacerbated by the requirement of shallow circuit depth necessary for their hardware implementation. Hybrid methods employing classical computers alongside quantum devices, such as the Variational Quantum Eigensolver (VQE), have proven useful for analyzing the capabilities of NISQ devices to solve relevant optimization problems. Still, in the simulation of complex structures involving the many-body problem in quantum mechanics, major issues remain about the representation of the system and obtaining results which clearly outperform classical computational devices. In this research contribution we propose the use of parameterized Tensor Networks (TNs) to attempt an improved performance of the VQE algorithm. A joint approach is presented where the Hamiltonian of a system is encapsulated into a Matrix Product Operator (MPO) within a parameterized unitary TN hereby splitting up the optimization task between the TN and the VQE. We show that the hybrid TN-VQE implementation improves the convergence of the algorithm in comparison to optimizing randomly-initialized quantum circuits via VQE.

==> content/extra_method.tex <==
Since TN can be used to envision complex interactions in a straightforward manner, they are great tools to represent quantum states. TN methods are able to capture the relevant entanglement properties of a quantum system, including its geometry and interactions. They provide an important analytic framework to understand the universal properties of different classes of states and their particular structures. The patterns they provide can be used to train computers, so they can obtain an appropriate initial state rather than randomly-initialized quantum circuits. This way maintaining a shallower circuit depth, yet increased expressivity.

%There are as many proposals as cases to be studied \citep{2017arXiv170903489H,2019NatCo..10.3007G,2020Quant...4..324L, 2021QS&T....6a4004K}, however TNs have shown great success when simulating ground states of Hamiltonians. Additionally, their patterns allow for a compact way of maintaining the complexity of the interactions being represented. The study of electronic structures as molecular Hamiltonians is a core matter in quantum chemistry, being of great relevance for drug discovery and chemical engineering among others \citep{2022PhR...986....1T}. 

%The idea behind this approach is based on the ability of TN methods to capture the relevant entanglement properties of the quantum system, including its geometry and interactions. The pattern provided by the TN ansatz can obtain an appropriate initial state, rather than utilizing randomly-initialized quantum circuits. Hence maintaining a shallower circuit depth, yet increased expressivity.
\\
A common approach is to choose an ansatz based on its ease of implementation on NISQ hardware.
Despite of the versatility and practicality of such an approach, once the circuits run on more than a few qubits, issues with optimization arise.
The dimension of the Hilbert space represented by the qubits scales exponentially with the number of qubits and an optimization method such as gradient descent is incapable of exiting the barren plateau on a quantum device within polynomial time \citep{2018NatCo...9.4812M}.

%Each \(W^{[i]}\) represents a 3 × 3 × 2 × 2 tensor(3 × 2 × 2 for \(W^{[1]}\) and \(W^{[n]}\)) with two dangling legs and two contracted legs that connect to the neighboring blocks

%Boundaries condition, where $W^{i_1, i'^1}$ and $W^{i_N, i'^N}$ are again row and column vectors.
%As Periodic Boundary conditions are applied, the top, $(W^{[1])}$, and bottom, $(W^{[n])}$, tensors are connected to each other.

%MPO Hamiltonians using Numpy
%\url{https://github.com/cmendl/pytenet/blob/master/pytenet/hamiltonian.py}

%Number of sites is n. (Please check.)

%\citep{roberts2019tensornetwork}
%Bond dimension is hard coded in this implementation.

%Starting from the transformation of the problem Hamiltonian to an MPO, which also entailed a unitary transformation.
%The unitary TN (uTN) surrounds the MPO Hamiltonian ensuring an overall simpler TN pattern to implement, while keeping the right energy values of the system.
%The problem Hamiltonian can be decomposed into Pauli coefficients, which is necessary for the connection to the VQE circuit since quantum devices are a 2-level system.

%One-dimensional
%MPS are efficient for simulating one-dimensional quantum systems and can represent a wide variety of one-dimensional quantum states.

%Two-dimensional
%MPO are two-dimensional tensor networks that represent a quantum operator by a sequence of tensors, where each tensor corresponds to an operator acting on two sites.

%One-dimensional
%MPO are used to efficiently represent operators for one-dimensional quantum systems and to perform simulations and calculations.
%MPO may provide a better chance at representing more complex systems, even if still 1D?
%\citep{2022arXiv221210421H}

%%Noise and it's effects
Aside from improving the trainabililty/optimization aspect, the use of TN can also benefit the implementation into NISQ hardware.  This noise flattens the cost function landscape E($\theta$). Without methods that reduce the effect of noise, VQE circuits have depths limited by the gate-error probability $p$ as $O(p-1)$. \cite{}

%issue arises in the energy landscape E($\theta$) when running the optimization scheme: Barren plateaus (vanishing gradients) appear if the Ansatz is unrelated to the Hamiltonian.
%Considering the limitations of NISQ devices, both in the number of qubits and the attainable circuit depths, this tends to be the case. Therefore preventing the scaling of the hardware-efficient ansatz used in previous experimental demonstrations \citep{dalton2022variational}. 

%These struggles lead to barren plateaus when running optimization schemes \citep{2018NatCo...9.4812M}.

%Barren plateaus occur mainly due to the randomness of the initial ansatz VQE are initiated from, thus if a better starting point is to be provided, they can be avoided. The proposal that is explored in this chapter is to use a Tensor Network as the initial ansatz from which to start the optimization of the quantum circuit implemented through the VQE.

%The development in quantum hardware has motivated the study of algorithms that are viable to run in the current NISQ devices. The most promising results in such regime have been hybrid quantum-classical algorithms, in which a parameterized quantum circuit is trained with a classical optimization loop. Among these, VQE has become a popular choice given its particularly good resilience to noise when implemented in quantum hardware \citep{2022PhR...986....1T}. 

%The compression scheme to encode the many-body 1D Hamiltonian is based on the image compression method of Singular Value Decomposition (SVD), in which a matrix gets decomposed in three matrices ($U, \Lambda, V^\dagger$), where the middle  one is a diagonal matrix with singular values. Thus, the decomposition is performed for each possible configuration, where an $i_n$ gets singled out from the rest of states while the diagonal matrix gets absorbed. This leaves two matrices, one for the single $i_n$ and the other with the rest of states. The approach is repeated until there is a matrix $A$ for each $i_n$. Thus, the wavefunction can be rewritten as:

. the Heisenberg magnet described by a nearest neighbor Hamiltonian along a chain of $N$ sites with periodic boundary condition has been really successful at providing insights on many-body problems

%These are known as Matrix Product Operators (MPOs) \citep{Solanki_2023}. The numerical simulations of many-body quantum systems based on matrix product states (MPS) and their generalization as Matrix Product Operators (MPO), have given good approximation results for 1D systems \citep{Nagy_2011,Dalzell_2019}.

%PERIODIIIIIIICC
When considering PBCs, the MPS ansatz turns into:
\begin{equation}
    |\psi\rangle = \sum_{i_1 , i_2...i_N} Tr(A^{i_1}A^{i_2}...A^{i_N})|i_1 i_2...i_N\rangle
\end{equation}

Similarly, the expression for an operator acting on a closed chain is of the form:
\begin{equation}\label{eq:MPO_periodic}
    O = \sum_{i_1 , i_2...i_N}\sum_{i'^1 , i'^2...i'^N} Tr\left( W^{i_1, i'1} W^{i_2,i'2}... W^{i_N,i'N}\right)|i_1,i_2...i_N\rangle \langle i'_1 i'_2...i'_N|
\end{equation}

Yet closing up the chain, where the edge particles also interact with each other, is an approach when constructing the TN structure to avoid having additional spin degrees of freedom dangling at the edges of the TN structure.
In this way the dangling legs of the TN are only of dimension $d$ as the local Hilbert space, and none $m$ dimension legs of the bonding are left to be considered.
In this work the systems discussed are assumed to be closed chains.

%%Periodic systems
%Until now, the boundary conditions of these matrix product states and operators have not been discussed. Returning once again to figure \ref{fig:MPS} where the decomposition of the many-body wavefunction is illustrated, one can notice that the $\alpha$ index appears at both ends of the diagram. 

%The ground state energy of the infinite system at criticality is -4/pi. As a convention one defines \(\sigma_z=diag([-1,1])\).

%The Hamiltonian can be decomposed into an MPO with Periodic Boundary Conditions, as seen in equation \ref{eq:MPO_periodic} and visually portrayed in figure \ref{fig:MPO_decomposition}. The matrices in the MPO in the case of the Transverse-Field Ising Model are the following:

%Old abstract-----------------------
Despite the advantage quantum computers are expected to deliver when performing simulations compared to their classical counterparts, the current noisy intermediate-scale quantum (NISQ) devices remain limited in their expressivity. The training of parameterized quantum circuits keeps being a significant practical challenge, exacerbated by the requirement of shallow circuit depth necessary for their implementation in NISQ devices.
Hybrid approaches employing classical computers alongside quantum devices, as the Variational Quantum Eigensolver (VQE), have proven efficient when tackling relevant optimization problems. However, one of the main challenges to this technique is the barren plateaus that occur when optimizing randomly-initialized quantum circuits. To tackle this phenomenon and improve the quantum many-body problems simulations, we propose the use of parametrized Tensor Networks (TN) within the VQE framework. TN can provide patterns to encapsulate deeper circuits without requiring a quantum computer to realize them. Matrix Product States (MPS) and Matrix Product Operators (MPOs) have given the best numerical results, as well as computational efficiency. In this chapter we will describe a joint approach where the Hamiltonian of a system will be parameterized by a unitary TN, in order to provide a reference for the quantum circuit from the VQE algorithm, and therefore converge to an improved result while keeping shallow quantum circuits.
%--------------------------------------------------------

%\subsection{Parallel circuits}
%TN-VQE involves the execution of many independent quantum circuits, which can be run simultaneously, either on different devices or on different sets of qubits within the same device. Doing so is beneficial because it reduces the amount of time needed to execute all the necessary circuits.

% Challenge of limited amount of qubits per device, and error propagation for complex circuits in NISQ devices.
% Parallel circuits implementation to TN ansatz to check to evaluate if different results will occur, and check the optimization efficiency

% Current quantum chips give reliable results only when executing a small circuit with shallow depth, causing a waste of hardware resources.
% Moreover, there is a growing demand to access quantum devices via the cloud, which leads to a large number of jobs in the queue and long waiting times for users. For example, it takes several days to get the result if we submit a circuit on IBM public quantum chips. Therefore, how to efficiently make use of quantum hardware to reduce the total runtime of circuits is becoming a timely problem

%The experiments of investigating parallel circuit execution on VQE and ZNE error mitigation method demonstrate how it can be useful for NISQ computing.
%\citep{DBLP:journals/corr/abs-2112-00387}
%\subsection{Circuit patchwork with tensor networks}
%Since the quantum circuits that we are able to run are limited in size, it is desirable to find a way to simulate larger problems without increasing the size of the required circuits. We propose a method for this which we will involve creating a patchwork of quantum circuits, connected by a tensor network.\\
%\\
%Consider a Hamiltonian with $m$ terms defined on $2N$ qubits:
%\[
%\hat{H}=\sum_{m=1}^Mc_m\bigotimes_{n=1}^{2N}\hat{\sigma}_m^n
%\]
%where $c_m$ are real valued coefficients and each $\hat{\sigma}_m^n$ is one of the three Pauli operators or the identity operator. Instead of using one circuit with $2N$ qubits, we can use two smaller circuits each with $N$ qubits. To do this
%We can partition the terms in the sum into three sets $S_1$, $S_2$ and $S_{12}$:
%\begin{enumerate}
%    \item The set $S_1$ consists of the values of $m$ in which the tensor product has Pauli operators only on the first $n_1$ qubits: $S_m = \{m | \forall n>N : \hat{\sigma}_m^n = \hat{I}\}$
%    \item The set $S_2$ consists of the values of $m$ in which the tensor product has Pauli operators only on the last $n_2$ qubits: $S_m = \{m | \forall n\leq N : \hat{\sigma}_m^n = \hat{I}\}$
%    \item The set $S_{12}$ contains all remaining terms: $S_{12} = \{m|m\notin (S_1 \cup S_2)\}$
%\end{enumerate}
%The Hamiltonian will then read:
%\[
%\hat{H}=\sum_{m}^{S_1}c_m\left(\bigotimes_{n=1}^{N}\hat{\sigma}_m^n\right)\otimes\hat{I}^{\otimes N}+\sum_{m}^{S_2}c_m\hat{I}^{\otimes N}\otimes\left(\bigotimes_{n=1}^{N}\hat{\sigma}_m^n\right)+\sum_{m}^{S_{12}}c_m\bigotimes_{n=1}^{2N}\hat{\sigma}_m^n
%\]
%Let the ansatzes of the two circuits be described with the unitaries $U(\phi_1)$ and $U(\phi_2)$ respectively, and let the tensor network unitary be $U(\theta)$. The expectation value is
%\[
%\braket{H} &= ...\\ 
%\]





\begin{enumerate}
\item Formulate problem Hamiltonian
\\
Finite transverse field Ising model
\begin{equation}
H = - J \sum_{i,j} \sigma^z_i \sigma^z_j - B \sum \sigma^x_i
\end{equation}
\\
The famous transverse field Ising Hamiltonian
The ground state energy of the infinite system at criticality is -4/pi.
\\
Convention: \(\sigma_z=diag([-1,1])\)
\\
Jx:  The Sx*Sx coupling strength between nearest neighbor lattice sites.
\\
Bz:  Magnetic field on each lattice site.

Question mark: \(J*g = B\)?

With the uTN structure, we can express the similarity transformation of a unitary
operator U on a Hamiltonian H, in tensor network diagrams:
\begin{equation}
H_{TN}= U^{\dagger}(\theta)H_{MPO}U(\theta)
\end{equation}\label{eq:UHU}

\\

\item Translate Hamiltonian from Pauli matrices to MPO representation:

For the example using the Ising Model the decomposition would be of the form:
\begin{equation}
H = H_{MPO} = J \prod_i^n W^{[i]}
\end{equation}

\begin{equation}
W^{[1]} = \begin{pmatrix}I_1 & -\sigma_z^1 & g \sigma^x_1\end{pmatrix}
\end{equation}
where  \(g=B/J\)?, three legs, 3x2x2

\begin{equation}
W^{[i]} = \begin{pmatrix}
I_i & -\sigma_z^i & g \sigma_x^i \\
0 & 0 & \sigma_z^i \\
0 & 0 & I_i \\
\end{pmatrix}
\end{equation}
four legs, 3x3x2x2

\begin{equation}
W^{[n]} = \begin{pmatrix}I_n & -\sigma_z^n & g \sigma^x_n\end{pmatrix}^T
\end{equation}
three legs, 3x2x2
\\
n blocks, each of which is a 3 × 3 matrix with 2 × 2 matrices as elements, and is denoted by \(W^{[i]}\) for \(i = 1,2,...,n\).

And \(I_i\), \(\sigma_i^x\), \(\sigma_i^y\), and \(\sigma_i^z\) are the identity and Pauli-X, Pauli-Y and Pauli-Z operators on the i-th qubit.
\\
Each \(W^{[i]}\) represents a 3 × 3 × 2 × 2 tensor
(3 × 2 × 2 for \(W^{[1]}\) and \(W^{[n]}\)) with two dangling legs
and two contracted legs that connect to the neighboring blocks

These $W^{[i]}$ matrices are a decomposition of the Hamiltonian operator, following a similar procedure to that of equation \ref{eq:MPS} \citep{Solanki_2023}. Given that operators in matrix representation have two indices, row and column, operators will also have two indices:
\begin{equation}
    H_{MPO} = \sum_{i_1 , i_2...i_N}\sum_{i'_1 , i'_2...i'_N} W^{i_1, i'^1}W^{i_2, i'^2},...W^{i_N, i'^N}|i_1,i_2...i_N\rangle \langle i'_1,i'_2...i'_N|
\end{equation}
the equation above corresponds to the MPO representation of a Hamiltonian with Open Boundaries condition, where $W^{i_1, i'^1}$ and $W^{i_N, i'^N}$ are again row and column vectors.
Meanwhile, for the Periodic Boundary conditions, the $H$ operator, is as follows:
\begin{equation}
    H_{MPO} = \sum_{i_1 , i_2...i_N}\sum_{i'_1 , i'_2...i'_N} Tr(W^{i_1, i'^1}W^{i_2, i'^2},...W^{i_N, i'^N})|i_1,i_2...i_N\rangle \langle i'_1,i'_2...i'_N|
\end{equation}

In this case, Periodic Boundary conditions are applied, meaning the top, $(W^{[1]}$, and bottom ,$(W^{[n]}$, tensors are connected to each other.
\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figures/H_mpo.png}
    \caption{This is the decomposed $H_{MPO}$ for the Ising model with 4 qubits. Given the Periodic Boundary conditions, the top and bottom are connected to each other.}
    \label{fig:H_wmatrices}
\end{figure}
\\

MPO Hamiltonians using Numpy
\url{https://github.com/cmendl/pytenet/blob/master/pytenet/hamiltonian.py}
\\
Number of sites is n. (Please check.)

Bond dimension equal to 2 for the physical inputs and outputs, but higher in the virtual bonds connectind the nodes forming the Hamiltonian MPO.

Connect start to end, so that there are none non-physical legs left dangling of the MPO structure.

\citep{roberts2019tensornetwork}
Bond dimension is hard coded in this implementation.

%Now, to consider an MPO \textit{O}, acting on $N$ sites, meaning number of tensors/nodes within the network, the matrix product form would be given by:
%\begin{equation}\label{eq:MPO}
%O^{j_1j_2...j_N}_{i_1i_2...i_N} = Tr(M^{j_1i_1} M^{j_2 i_2} ... M^{j_N i_N} )
%\end{equation}
%where $M^{j_k i_k}$ is a $D \times D$ matrix, where $i_1 i_2 ... i_N$ and $j_1 j_2 ...j_N$ are the labels for the physical legs \citep{_ahino_lu_2018}.

\\
\item Choose tensor network unitary U($\theta$) 

The matrix of choice is a special case of the arbitrary rotation one shown in equation \ref{eq:arbitrary_matrix}. This matrix is known as the phase shift gate matrix and is parameterised by a single angle:
\begin{equation}
R(\theta_1)=
\begin{bmatrix}
    e^{-i\theta_1}  & 0 \\
    0   & e^{i\theta_1} 
\end{bmatrix}
\end{equation}
From the tensor product of this unitary matrix, an MPO, which is a generalization of a matrix product representation to the operator space, is obtained:
\begin{equation}
M^{ijkl}(\theta) = R(\theta)^{ij} \otimes R(\theta)^{kl}
\end{equation}\label{eq:single_mpo}

This results in an MPO of dimensions $2 \times 2 \times 2 \times 2$. These are the desired dimensions to be assembled in a symmetric network that will have as many physical input and output legs as the Hamiltonian size requires, while keeping the bond dimension at 2. The test to prove that this MPO is unitary is explained in depth in section \ref{sec:unitary_check}. 
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/uMPO.png}
    \caption{This is the structure of the uMPO attached at each end of the Hamiltonian ($U^{\dagger}(\theta)HU(\theta)$). Each of the boxes is a unitary MPO obtained from equation \ref{eq:single_mpo}, $M^{ijkl}(\theta)$ in the case of $U(\theta)$ and $M^{\dagger jilk}(\theta)$ for the $U^{\dagger}(\theta)$ network. The dimensions of each physical input and output is of order 2.}
    \label{fig:U_theta}
\end{figure}
Once a unitary $M^{ijkl}(\theta)$ has been constructed as prescribed, the next step is to build the symmetric uMPO network by connecting a set of $M^{ijkl}(\theta)$ to each other. In the example treated here with 4 qubits, the desired number of input and output physical legs is 4 as well. The construction followed is illustrated in figure \ref{fig:U_theta}, where five $M^{ijkl}(\theta)$ are connected to build a symmetric uMPO  matching the size of the Hamiltonian. This structure will be denoted as $U(\theta)$, in which $\theta$ is a vector containing as many parameters as the unitary matrix in equation \ref{eq:single_mpo} requires. 

In order to perform the unitary transformation from equation \ref{eq:UHU} representing the problem Hamiltonian through uTN, $U^{\dagger}(\theta)$ is required. The procedure to build the latter is the same as for $U(\theta)$, only that the network is built with $M^{\dagger jilk}(\theta)$ as the tensors.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/contraction_leg.png}
    \caption{The figure depicts the Einstein summation behind the contraction of each connecting leg between tensors in figure \ref{fig:U_theta}. Therefore, there would be 6 contractions of this type to obtain the parameterised contracted uTN $U(\theta)$.}
    \label{fig:leg_contraction}
\end{figure}

First all the edges need to be connected, following the design in Figure \ref{fig:U_theta}, so that a network contractor can be applied to all the connections. The \textit{contractors.auto()} function from from the \textit{TensorNetwork} package is used here \citep{roberts2019tensornetwork}. This function uses Einstein summation to contract over the connected edges of the tensors provided as inputs. As shown in figure \ref{fig:leg_contraction}, each leg between two tensors (nodes) will be contracted. In this case, there is a total of 6 contractions, which are summed over to obtain the resulting uTN.

In addition, the order of the output edges also needs to be specified, and needs to be remembered to keep track of how to connect in further contractions. Since all the edges have the same dimension, these actions can be encapsulated in loops that iterate over the connections and leftover edges. 
\\
%\url{https://authors.library.caltech.edu/83074/2/PhysRevB.98.245122.pdf}
%\url{https://link.springer.com/chapter/10.1007/978-3-030-34489-4_2}

%\url{https://arxiv.org/pdf/2009.02606.pdf}
%\url{https://arxiv.org/pdf/1506.07179.pdf}

%Once a unitary $M^{ijkl}(\theta)$ has been constructed as prescribed, the next step is to build the symmetric uMPO network by connecting a set of $M^{ijkl}(\theta)$ to each other. In the example treated here with 4 qubits, the desired number of input and output physical legs is 4 as well. The construction followed is illustrated in figure \ref{fig:U_theta}, where five $M^{ijkl}(\theta)$ are connected to build a symmetric uMPO  matching the size of the Hamiltonian. This structure will be denoted as $U(\theta)$, in which $\theta$ is a vector containing as many parameters as the unitary matrix in equation \ref{eq:single_mpo} requires. 

\item Combine Hamiltonian and U($\theta$) to get TN:

Three different tensor networks have been built til this point: $U(\theta)$, $H_{MPO}$ and $U^{\dagger}(\theta)$. They all need to be connected to obtain $H_{TN}$ from the equation \ref{eq:UHU}. The way their legs are connected is shown in figure \ref{fig:UHU}.
The contraction between the virtual bonds, connecting legs between the three nodes, are once again through Einstein summation as explained before in figure \ref{fig:leg_contraction}.

\\

%First all the edges need to be connected, following the design in Figure \ref{fig:U_theta}, so that a network contractor can be applied to all the connections. Contraction between the tensors represents summation. Thus, the \textit{contractors.auto()} function from from the \textit{TensorNetwork} package used here \citep{roberts2019tensornetwork} uses Einstein summation to contract over the connected edges of the tensors provided as inputs. As shown in figure \ref{fig:leg_contraction}, each leg between two tensors (nodes) will be contracted. In this case, there is a total of 6 contractions, which are summed over to obtain the resulting uTN.

%In addition, the order of the output edges also needs to be specified, and needs to be remembered to keep track of how to connect in further contractions. Since all the edges have the same dimension, these actions can be encapsulated in loops that iterate over the connections and leftover edges. 


%Since we know that \(\hat{O}^{\dagger}\hat{O} = \hat{I} ^{\otimes N}\) for all system sizes, each of the operators $\hat{O}$ must be individually equal to $\hat{I}$. \ref{}

%Only one block of these operators can have diagonal terms, since otherwise it would imply that \(O^{\dagger}O\) is only proportional to I$\otimes$N and it is not possible to normalize the expression to make it exactly equal to I$\otimes$N.

%To accomodate for the above, one can choose a unitary tensor network with the same bond dimension as the Hamiltonian and size of network is equal to number of sites n. This has to be re-formulated with respect to size of the network in horizontal and vertical direction and is therefore dependent on the Hamiltonian taken under consideration.
\\

\item Contract TN to calculate traces for Pauli coeffs.

The VQE requires measuring in the Pauli basis, reason why the Pauli decomposition of $H_{TN}(\theta)$ is considered to calculate the energy of the system. The resulting energy can be expressed as a linear combination of expectation values:
\begin{equation}
    E(\theta, \phi)= \sum_P c_P (\theta) \langle P \rangle_{\phi}
\end{equation}
the coefficients $c_P (\theta)$ are obtained by tracing the TN with possible Pauli string combinations:
\begin{equation}
    c_P (\theta)= Tr[ P U^{\dagger}(\theta)H U(\theta)]
\end{equation}\label{eq:cp}
The trace of a tensor, as illustrated in figure \ref{fig:trace}, is obtained by connecting the tensor with itself. Therefore, to calculate the $c_P (\theta)$ coefficients, the left and right edges in the structure from figure \ref{fig:paulis} are connected with each other for each of the Pauli combinations.
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/trace.png}
    \caption{The figure depicts the operation of tracing a matrix $R^{ij}$, which in tensor network diagrams is equivalent to contracting the tensor with itself.}
    \label{fig:trace}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/paulis_hTN.png}
    \caption{This is the set up to calculate the $c_P (\theta)$ coefficients, where $\sigma_i, \sigma_j, \sigma_k, \sigma_l $ are Pauli matrices. All different combinations of Pauli matrices are considered, discarding the ones resulting in zero traces.}
    \label{fig:paulis}
\end{figure}

The physical inputs and outputs of the TN are of dimension 2, therefore the Pauli strings to be attached at their ends would be of that same dimension. There are 4 wires in our $H_{TN}$, and each possible combination of Pauli operators needs to be measured in order to obtain the energy. Luckily, some of the combinations have a zero traces that can be discarded.
\\

\item Reconstruct new Hamiltonian
- Add results of contractions
\\
\item Quantum circuit U(phi)

Define circuit.

In principle, the structure of the parameterised quantum circuit $U(\phi)$ can be arbitrary.
\\

\item Optimize the parameters theta and phi with VQE sequentially or in parallel.

The minimization problem to be solved by VQE assisted with $H_{TN}$:
\begin{equation}
    min_{\theta, \phi} \langle 0| U^{\dagger}(\phi)U^{\dagger}(\theta) HU(\theta)U(\phi)|0\rangle
\end{equation}

When freezing the TN vector $\theta$, then the problem becomes a traditional VQE problem. While if the quantum circuit parameter $\phi$ is frozen, then a classical gradient descent to optimize $H_{TN}$ using the formula:
\begin{equation}
    \frac{\partial E (\theta, \phi)}{\partial \theta}= Tr(\frac{ P U^{\dagger}(\theta)H U(\theta)}{\partial \theta})
\end{equation}
\end{enumerate}


\subsection{Algorithm}

\section{Experimental Study}
\subsection{Overview of simulation study}
Despite the advantage quantum computers are expected to deliver when building simulations compared to their classical counterparts, the current noisy intermediate-scale quantum (NISQ) devices remain limited in their expressivity. The training of parametrized quantum circuits keeps being a significant practical challenge, exacerbated by the requirement of shallow circuit depth necessary for their implementation in NISQ devices.

Hybrid approaches employing classical computers alongside quantum devices, as the Variational Quantum Eigensolver (VQE), have proven efficient when tackling relevant optimization problems. However, one of the main challenges to this technique is the barren plateaus that occur when optimizing randomly-initialized quantum circuits. To tackle this phenomenon and improve the quantum many-body problems simulations, we propose the use of parametrized Tensor Networks (TN) within the VQE framework. TN can provide patterns to encapsulate deeper circuits without requiring the computer to realize them. From which Matrix Product States (MPS) and Matrix Product Operators (MPOs), have given the best numerical results, as well as computational efficiency. In this chapter we will describe a joint approach where the Hamiltonian of a system will be parametrized by a unitary TN, in order to provide a reference for the quantum circuit from the VQE algorithm, and therefore converge to an improved result while keeping shallow quantum circuits.

\subsection{Consistency checks}
\subsubsection{TN unitarity check}\label{sec:unitary_check}
For \textit{O} to be unitary, it would have to satisfy that $O^{\dagger}O = I$. O can be called a matrix product unitary operator if it is a unitary for all system sizes. So going back to the matrix product form of \textit{O}, where \textit{M} can be understood as a finite-bond dimension tensor representing \textit{O}. We can use the elements of \textit{M} tensor, which are the matrices $M^{j_k i_k}$ to check the MPO construction is unitary.

The elements of the $M^{\dagger}$ tensor needed to proved the identity, are obtained from the $M^{ij}$ matrices using:
\begin{equation}
M^{\dagger^{ji}} = (M^{ij})^*
\end{equation}\label{eq:dagger_M}
Then, we can check the unitary constrain by a composite of the $O^{\dagger}O $ operation of the form:
\begin{equation}
T^{ij} = \sum_k M^{\dagger ik} \otimes M^{kj}
\end{equation}\label{eq:composite}
If \textit{O} is to be unitary, the tensor $T^{ij}$ should be equivalent to a tensor product of identity operators.

The next step was to check $M^{ij}(\theta)$ was indeed a unitary tensor. To do so, we reference back to equation \ref{eq:composite} where through calculating the composite, one could confirm the tensor was unitary if the identity operators were obtained as a result. Our MPO satisfied such requirements, achieving the following results:
\begin{equation*}
M^{\dagger ji}(\theta) \otimes M^{ij}(\theta) = I^{ij} \otimes I^{ij}
\end{equation*}
\begin{equation}
M^{\dagger ji}(\theta) \cdot M^{ij}(\theta) = I^{ij}
\end{equation}

==> content/instructions_references.tex <==
%\begin{thebibliography}{}
 
 %\bibitem[Huang, J. et al (2022)]{HUA22}
 %Huang, J. and He, W. and Zhang, Y. and Wu, Y. and Wu, B. and Yuan, X. (2022). Tensor Network Assisted Variational Quantum Algorithm. \emph{arXiv e-prints}. doi:10.48550/arXiv.2212.10421

%\bibitem[Roberts, C. et al (2019)]{tn19}
 %Roberts, C., Milsted, A., Ganahl, M., Zalcman, A., Fontaine, B. Zou, Y., Hidary, J., Vidal, G., \& Leichenauer, S. (2019). TensorNetwork: A Library for Physics and Machine Learning. \emph{arXiv:1905.01330}

%\bibitem[Solanki, P. D., \& Ramkarthik, M. S. (2023)]{SOL23}
 %Solanki, P. D., \& Ramkarthik, M. S. (2023). A new general approach for obtaining matrix product operators for spin Hamiltonians with periodic boundary conditions. \emph{ Physica Scripta, Volume 98}. doi:10.1088/1402-4896/acb5cf



%\bibitem[Schatz(2000)]{Sch00}
%Schatz, B.~R. (2000, November 17). Learning by text or context? [Review of the
% book \emph{The social life of information}, by J.~S. Brown \& P. Duguid].
%\emph{Science}, \emph{290}, 1304.

%\bibitem[Schwartz(1993)]{Sch93}
%Schwartz, J. (1993, September 30). Obesity affects economic, social status.
% \emph{The Washington Post}, pp.~A1, A4.

%\bibitem[Von~Ledebur(2007)]{VL07}
%Von~Ledebur, S.~C. (2007). Optimizing knowledge transfer by new employees in
% companies. \emph{Knowledge Management Research \& Practice}. Advance online
 %publication. doi:10.1057/palgrave/kmrp.8500141

%\end{thebibliography}

\bigskip
\noindent Each entry takes the form:
\begin{verbatim}
\bibitem[short list of authors' surnames(date of publication)long list
 of authors' surnames]{key}
Bibliography entry
\end{verbatim}
where `\texttt{long list of authors' surnames}' is the \emph{optional} `long' list of three, four or five names which enables them all to appear where the \verb"bibitem" is first cited in the text (if the long list is missing, the short list will be used instead), and `\texttt{key}' is the tag that is to be used as an argument for the \verb"\cite" commands in the text of the article. `\texttt{Bibliography entry}' is the material that is to appear in the list of references, suitably formatted. The commands
\begin{verbatim}
\usepackage[longnamesfirst,sort]{natbib}
\bibpunct[, ]{(}{)}{;}{a}{,}{,}
\renewcommand\bibfont{\fontsize{10}{12}\selectfont}
\end{verbatim}
need to be included in the preamble of your .tex file in order to generate the citations and bibliography as described above.

Instead of typing the bibliography by hand, you may prefer to create the list of references using a \textsc{Bib}\TeX\ database. For this we suggest using Erik Meijer's \texttt{apacite} package, which is available via CTAN if you do not already have it. The \verb"apacite.sty", \verb"apacite.bst" and (if your paper is written in English) \verb"english.apc" files need to be in your working folder or an appropriate directory, the commands
\begin{verbatim}
\usepackage[natbibapa,nodoi]{apacite}
\setlength\bibhang{12pt}
\renewcommand\bibliographytypesize{\fontsize{10}{12}\selectfont}
\end{verbatim}
included in the preamble of your .tex file instead of the \verb"\usepackage[]{natbib}", \verb"\bibpunct" and \verb"\renewcommand\bibfont" commands described above, and the lines
\begin{verbatim}
\bibliographystyle{apacite}
\bibliography{interactapasample}
\end{verbatim}
included where the list of references is to appear, where \texttt{interactapasample.bib} is the bibliographic database included with the \textsf{Interact}-APA \LaTeX\ bundle (to be replaced with the name of your own .bib file). The \verb"[natbibapa]" option has to be added to \verb"\usepackage{apacite}" in order to enable citation commands of the type \verb"\citep" and \verb"\citet". \LaTeX/\textsc{Bib}\TeX\ will extract from your .bib file only those references that are cited in your .tex file and list them in the References section.

Please include a copy of your .bib file and/or the final generated .bbl file among your source files if your .tex file does not contain a reference list in a \texttt{thebibliography} environment.


